Play Guessing Game with LLM: Indirect Jailbreak Attack with Implicit Clues

With the development of LLMs, the security threats of LLMs are getting more and more attention. Numerous jailbreak attacks have been proposed to assess the security defense of LLMs. Current jailbreak attacks primarily utilize scenario camouflage techniques. However their explicitly mention of malicious intent will be easily recognized and defended by LLMs. In this paper, we propose an indirect jailbreak attack approach, Puzzler, which can bypass the LLM's defense strategy and obtain malicious response by implicitly providing LLMs with some clues about the original malicious query. In addition, inspired by the wisdom of "When unable to attack, defend" from Sun Tzu's Art of War, we adopt a defensive stance to gather clues about the original malicious query through LLMs. Extensive experimental results show that Puzzler achieves a query success rate of 96.6% on closed-source LLMs, which is 57.9%-82.7% higher than baselines. Furthermore, when tested against the state-of-the-art jailbreak detection approaches, Puzzler proves to be more effective at evading detection compared to baselines.

==> tab/RQ1_maliciousdata.tex <==
\begin{table}[t]

% \Huge
  \caption{The quality and the query success rate of the jailbreak prompts generated by {\tool} and baselines}
  \label{tab:RQ1_performance_maliciousdata}
  % * indicates that the model is trained on the source domain, and the value in ( ) indicates the proportion of training data in the training set.
  
\resizebox{0.5\textwidth }{!}{
\begin{threeparttable}
\begin{tabular}{cc|ccccccc}
\toprule
\multirow{2}{*}{\textbf{Tested Model}} &
  \multirow{2}{*}{\textbf{Metric}} & 
  \multirow{2}{*}{\textbf{{\tool}}} &
  % \multirow{2}{*}{\textbf{MR3}} &
  % \multirow{2}{*}{\textbf{{\tool}}} &
  \multirow{2}{*}{\textbf{TAP}} &
  
  

  % \multirow{2}{*}{\textbf{SIN}} &
  \multicolumn{4}{c}{\textbf{HandCraft Prompts}}\\     \cline{5-7} 

 
   &
    &
    &
  % \multicolumn{1}{c}{\textit{\textbf{SwapAnt}}}  
     % \multicolumn{1}{c}{\textit{\textbf{SwapAnt}}} &
 
% \multicolumn{1}{c}{\textit{\textbf{MR-SS}}}  &
%      \multicolumn{1}{c}{\textit{\textbf{MR-NR}}} &
     &
   

  \multicolumn{1}{c}{\textit{\textbf{CR}}} &

  \textit{\textbf{TC}} &
  \multicolumn{1}{c}{\textit{\textbf{SIMU}}} &


  \\ \midrule
\multirow{2}{*}{{GPT3.5}} &
  \textit{QSR} &

  \multicolumn{1}{c}{\textbf{100\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{329} & 

   
 % \multicolumn{1}{c}{56\%} & 
  

90\% & 
  
 
  53\%&
   
  \multicolumn{1}{c}{40\%}  \\ 
  
&\textit{MatchRate} &

  \multicolumn{1}{c}{90.0\%} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{329} & 

    
%  \multicolumn{1}{c}{77.2\%} & 
  

  \textbf{93.6\%}  & 
  
  86.7\% &
   
  \multicolumn{1}{c}{90.9\%} \\ 


  
 

  
  
   \midrule
\multirow{2}{*}{{GPT4}} &
  \textit{QSR} &
\multicolumn{1}{c}{\textbf{100\%}} & 
  \multicolumn{1}{c}{0\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{50\%} & 

  
   13\%  &
  40\% &
   
  \multicolumn{1}{c}{\%} \\ 

    & \textit{MatchRate} &
\multicolumn{1}{c}{86.0\%} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{79.7\%} & 
  
  \textbf{84.6\%} & 
  
 
  85.0\% &
   
  \multicolumn{1}{c}{0.0\%}  \\ 


  \midrule
\multirow{2}{*}{{GPT4-Turbo}} &
  \textit{QSR} &
\multicolumn{1}{c}{\textbf{100\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{44\%} & 

  
   0\%  &
  7\% &
   
  \multicolumn{1}{c}{0\%}  \\ 

    & \textit{MatchRate} &
\multicolumn{1}{c}{\textbf{87.0\%}} & 
  \multicolumn{1}{c}{\%} & 

  
   0.0\% & 
  
 
  85.7\% &
   
  \multicolumn{1}{c}{0.0\%}  \\ 



  \midrule

\multirow{2}{*}{{Gemini-pro}} &
  \textit{QSR} &
\multicolumn{1}{c}{\textbf{83\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{44\%} & 

  
   47\%  &
  0\% &
   
  \multicolumn{1}{c}{17\%}  \\ 

    & \textit{MatchRate} &
\multicolumn{1}{c}{\textbf{86.7\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{84.0\%} & 
  
   89.3\% & 
  
 
  0.0\% &
   
  \multicolumn{1}{c}{88.2\%}  \\ 
  \midrule
  
  \multirow{2}{*}{{LLama-7B}} &
  \textit{QSR} &
\multicolumn{1}{c}{\textbf{3\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{44\%} & 

  
   0\%  &
  0\% &
   
  \multicolumn{1}{c}{0\%}  \\ 

    & \textit{MatchRate} &
\multicolumn{1}{c}{\textbf{66.7\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{84.0\%} & 
  
   0\% & 
  
 
  0\% &
   
  \multicolumn{1}{c}{0\%}  \\ 

 
  \midrule

  \multirow{2}{*}{{LLama-13B}} &
  \textit{QSR} &
\multicolumn{1}{c}{\textbf{29\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{44\%} & 

  
  0 \%  &
 0 \% &
   
  \multicolumn{1}{c}{0\%}  \\ 

    & \textit{MatchRate} &
\multicolumn{1}{c}{\textbf{100.0\%}} & 
  \multicolumn{1}{c}{\%} & 
  % \multicolumn{1}{c}{306} & 
   
   

%  \multicolumn{1}{c}{84.0\%} & 
  
   0\% & 
  
 
  0\% &
   
  \multicolumn{1}{c}{0\%}  \\ 

 

  



  
 

  \bottomrule
\end{tabular}
  \end{threeparttable}
        % \end{threeparttable}
}
\end{table}

==> tab/RQ2_offensiveprompt.tex <==
\begin{table}[t] \tiny
\caption{The quality and query success rate of the Offensive prompts generated by {\tool}.}
% \yang{comment.}}
% improved accuracy是不是不用单列一行，直接在retrained那个数值后面打个括弧，写上+XXX？
\label{tab:rq1}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc}
\toprule
\textbf{Metric} & \textbf{GPT3.5} & \textbf{GPT4} & \textbf{GPT4-Turbo} \\ \midrule

QSR &   100\%     &   99.8\%    &   95.6\%     \\
ToxicScore &   4.3     &   4.4    &   4.6     \\






\bottomrule
\end{tabular}
}
\end{table}
